Revisiting Adversarial Risk

Recent works on adversarial perturbations show that there is an inherent trade-off between standard test accuracy and adversarial accuracy. Specifically, they show that no classifier can simultaneously be robust to adversarial perturbations and achieve high standard test accuracy. However, this is contrary to the standard notion that on tasks such as image classification, humans are robust classifiers with low error rate. In this work, we show that the main reason behind this confusion is the inexact definition of adversarial perturbation that is used in the literature. To fix this issue, we propose a slight, yet important modification to the existing definition of adversarial perturbation. Based on the modified definition, we show that there is no trade-off between adversarial and standard accuracies; there exist classifiers that are robust and achieve high standard accuracy. We further study several properties of this new definition of adversarial risk and its relation to the existing definition.

==> adv_training.tex <==
In this section we study the properties of minimizers of objective~\eqref{eqn:objective_mod} and its relation to the commonly used adversarial training objective in Equation~\eqref{eqn:adv_obj}. Our main results in this section assume that the base classifier $g(x)$ is a Bayes optimal classifier. This is a reasonable assumption because in many classification tasks the labels are generated by humans (\textit{i.e.,} human is a Bayes optimal classifier for the classification task) and robustness is also measured w.r.t a human. The following Theorem shows that under this condition, the minimizers of \eqref{eqn:objective_mod} are Bayes optimal. 
\begin{theorem}
\label{lem:minimizers}
Suppose the hypothesis class $\mathcal{F}$ is equal to the set of all measurable functions. Let the base classifier $g(x)$ be a Bayes optimal classifier.
\begin{enumerate}
    \item (\textbf{$0/1$ loss}). If $\ell$ is the $0/1$ loss, then any minimizer $\hat{f}$ of $$\min_{f \in \mathcal{F}} R_{0-1}(f)+\lambda R_{\text{adv}, 0-1}(f),$$ is a Bayes optimal classifier.
    \item (\textbf{Logistic loss}). Suppose $\ell$ is the logistic loss, which is a convex surrogate of $0/1$ loss. Moreover, suppose the probability distribution $\mathcal{P}$ is such that $\left|\mathbb{P}(y = 1 | x) - \frac{1}{2}\right| > \gamma$ a.e., for some positive constant $\gamma$. Then any minimizer of Equation~\eqref{eqn:objective_mod} is a Bayes optimal classifier. 
\end{enumerate}
\end{theorem}
%This suggests that given huge amounts of training data, minimizing $R_n(f)$ over complex hypothesis space $\mathcal{F}$ should give us robust classifiers.
The first part of the above Theorem shows that minimizing the joint risk with $0/1$ loss, for any choice of $\lambda \geq 0$, results in a Bayes optimal classifier. This shows that Bayes optimal classifier is both robust and achieves high standard accuracy and there is no trade-off between adversarial and standard risks. The second part of the Theorem, which is perhaps the more interesting result, shows that using a convex surrogate for the $0/1$ loss to minimize the joint risk also results in Bayes optimal classifiers. This result assures us that optimizing a convex surrogate does not hinder our search for a robust classifier that has low adversarial and standard risks. 

%Finally, we note that the first part of the above Theorem can be extended to the setting where $\mathcal{F}$ is not the set of all measurable functions. By assuming that $\mathcal{F}$ contains a Bayes optimal classifier, we can show that the minimizer of .
We now briefly discuss the scenario where the base classifier $g(x)$ is not Bayes optimal. In this case, the first term in the joint objective will bias the optimization towards towards a Bayes optimal classifier. Whereas, the second term in the joint objective will bias the optimization towards the base classifier. Since the base classifier is not a Bayes optimal classifier, this results in a trade-off between the two terms, which is controlled by the tuning parameter $\lambda$. If $\lambda$ is small, then the minimizers of the joint objective will be close to a Bayes optimal classifier. If $\lambda$ is large, the minimizers will be close the base classifier.

As mentioned in the previous section, most of the existing works on adversarial robustness try to minimize the adversarial risk defined in Equation~\eqref{eqn:adv_obj}. We now show that the objective \eqref{eqn:adv_obj} is related to Equation~\eqref{eqn:objective_mod}, under certain assumptions on the Bayes decision rule $\eta(x) = \text{sign}(2\mathbb{P}(y = 1|x) - 1)$. Specifically, we show that when $\eta(x)$ satisfies a ``margin condition'', then minimizing objective~\eqref{eqn:adv_obj} also results in Bayes optimal classifiers.
\begin{theorem}
\label{lem:equiv}
Suppose the hypothesis class $\mathcal{F}$ is equal to the set of all measurable functions. Moreover, suppose the Bayes decision rule $\eta(x)$ satisfies the following margin condition: 
\begin{equation}
\label{eqn:margin}
\mathbb{P}_x\left(\exists \tilde{x} : \|\tilde{x} - x\| \leq \epsilon, \eta(\tilde{x}) \neq \eta(x)\right) = 0.
\end{equation}
Let $G_{\text{adv},0-1}(f)$ be the adversarial risk obtained by replacing $g(x)$ with $y$ in $R_{\text{adv},0-1}(f)$
\begingroup\makeatletter\def\f@size{9}\check@mathfonts
\[
G_{\text{adv},0-1}(f) = \mathbb{E}\left[ \sup_{\begin{subarray}{c} \|\delta\|\leq \epsilon \end{subarray}} \ell_{0-1}\left(f(x+\delta), y \right) - \ell_{0-1}\left(f(x), y \right) \right].
\]
\endgroup
Let $G_{\text{adv}}(f)$ denote the adversarial risk obtained by replacing $\ell_{0-1}$ in $G_{\text{adv},0-1}(f)$ with a convex surrogate loss $\ell$.
\begin{enumerate}
    \item (\textbf{$0/1$ loss}). If $\ell$ is the $0/1$ loss, then any minimizer of $$\min_{f \in \mathcal{F}} R_{0-1}(f)+\lambda G_{\text{adv}, 0-1}(f),$$ is a Bayes optimal classifier.
    \item (\textbf{Logistic loss}). Suppose $\ell$ is the logistic loss. Moreover, suppose the probability distribution $\mathcal{P}$ is such that $\left|\mathbb{P}(y = 1 | x) - \frac{1}{2}\right| > \gamma$ a.e., for some positive constant $\gamma$. Then any minimizer of 
    
\begin{equation}
\label{eqn:objective_standard}
\min_{f \in \mathcal{F}} R(f) + \lambda G_{\text{adv}}(f),
\end{equation}
is a Bayes optimal classifier
\end{enumerate}

%be obtained by replacing $g(x)$ in $R_{\text{adv}, 0-1}(f),$ with $y$
% Consider the following objective obtained by replacing $g(x)$ in $R_{0-1}(f)+\lambda R_{\text{adv}, 0-1}(f),$ with $y$.

% Then for any $\lambda \geq 0$, any minimizer $\hat{f}$ of objective~\eqref{eqn:objective_standard} is a Bayes optimal classifier. 
 
\end{theorem}
Note that, objective~\eqref{eqn:adv_obj} is equivalent to objective~\eqref{eqn:objective_standard} for $\lambda = 1$.
If $\eta(x)$ satisfies the margin condition, then Theorem~\ref{lem:equiv} shows that minimization of objective \eqref{eqn:adv_obj} results in a Bayes optimal classifier. It also shows that under the margin condition there is no trade-off between the older definition of adversarial risk and standard risk.

If $\eta(x)$ doesn't satisfy the margin condition, then the above results need not hold and  minimizers of~\eqref{eqn:objective_standard} need not be Bayes optimal. In fact, if the margin condition is violated, it is very easy to construct examples for which the minimizers of~\eqref{eqn:objective_standard} are not Bayes optimal. Below we consider concrete examples which don't satisfy the margin and show that minimizing~\eqref{eqn:objective_standard} leads to solutions with poor standard accuracy. This shows that the margin condition is a very important condition for Bayes optimality. 

In a recent work \citet{sharif2018suitability} try to estimate the margin in MNIST~\citep{lecun1998mnist}, CIFAR10~\citep{krizhevsky2009learning} datasets via user studies. Their results show that the margin in these datasets is smaller than the magnitude of adversarial perturbations used in prior works. Together with the above discussion on importance of margin, their results can potentially explain the drop in standard accuracy that has been observed on MNIST, CIFAR10 when performing adversarial training with large adversarial perturbations~\citep{madry2017towards, 2018arXiv180801688S}.

\paragraph{Synthetic Dataset.} We now consider a simple synthetic dataset to illustrate the importance of margin for objective~\ref{eqn:objective_standard}. Consider the following data generation process in a 2D space. The marginal distribution of $y$ is given by $\mathbb{P}(y = 1) = \frac{3}{4},\quad \mathbb{P}(y = -1) = \frac{1}{4}$, and the conditional distributions follow uniform distributions on squares of side length $2$ centered at $(-1.2, 0)$, $(1.2,0)$ respectively
$$\mathbb{P}\left(x - (1.2y, 0)|y\right) \sim U[-1,1]^2.$$ 
Let $\eta(x)$ be the Bayes decision rule
\[
\eta(x) = \begin{cases}1 & \text{if } x_1 \geq 0\\ -1 & \text{if } x_1 < 0\end{cases}.
\]
Note that the data is linearly separable and has a margin of $0.2$ w.r.t $L_{\infty}$ norm. From Theorem~\ref{lem:equiv} we know that for $L_{\infty}$ norm perturbations with $\epsilon \leq 0.2$, minimizing Equation~\ref{eqn:objective_standard} results in Bayes optimal classifiers. To verify this, we generated $10^5$ training samples from this distribution and minimized objective~\eqref{eqn:objective_standard} over 1 hidden layer feed forward networks with 100 hidden units. We used PGD training proposed by~\citet{madry2017towards} to minimize the objective. Figure~\ref{fig:toy} shows the behavior of standard risk of the resulting model, as we vary $\epsilon$. We can seen that for $\epsilon \leq 0.2$, the standard risk is zero. Whereas, for $\epsilon > 0.2$, the standard risk is non-zero.
% \begin{wrapfigure}{r}{0.4\textwidth}
% \centering
% \includegraphics[scale=0.3]{non-robust.png}
% \caption{One-dimensional mixture embedded in a 2-D space. Observe the classifier that is nearly parallel to the $x_1$ axis. Despite having low true risk, it will have high adversarial risk for a small $\epsilon$}
% \label{fig:robust}
% \end{wrapfigure}
\begin{figure}
\centering
\includegraphics[width=0.38\textwidth]{plots/toy.eps}
%\subfigure[\label{fig:cifar_pgd_lambda}]{\includegraphics[width=0.3\textwidth]{plots/cifar_pgd_lambda.eps}}
\vspace{-0.12in}
%\caption{Figure on the left shows Classification $0/1$ risk vs. $\epsilon$ on the synthetic dataset. Figure on right shows the behavior of various risks obtained by adversarial training with $\epsilon = 0.03$, with varying $\lambda$. The adversarial perturbations in both the experiments are measured w.r.t $L_{\infty}$ norm.}
\caption{Figure shows standard $0/1$ risk vs. $\epsilon$ on the synthetic dataset. The adversarial perturbations are measured w.r.t $L_{\infty}$ norm.}
\label{fig:toy}
\end{figure}

\paragraph{Choice of $\lambda$.} Existing works on adversarial training always choose $\lambda = 1$ for minimization of \eqref{eqn:objective_standard}. However we note that $\lambda = 1$ may not always be the optimal choice. Indeed $\lambda$ captures the tradeoff between two distinct objects: the classification risk, and the \emph{excess risk} due to adversarial perturbations, and it is thus quite natural to expect the optimal tradeoff to occur at values other than $\lambda = 1$.
Figure~\ref{fig:cifar_pgd_lambda} shows the behavior of various risks of models obtained by minimizing objective~\eqref{eqn:objective_standard} on CIFAR10, for various choices of $\lambda$. We use VGG11 network with reduced capacity, where we reduce the number of units in each layer to $1/4^{th}$.  We defer the details of the training procedure to the next section. It can be seen that as $\lambda$ increases adversarial risk goes down but classification risk goes up and an optimal choice of $\lambda$ should be based on the metric one cares about.
if one cares about the joint risk then $\lambda = 2$ has slightly better performance than $\lambda = 1$. In the experimental results we present in later sections, we also notice settings where the optimal choice of $\lambda$ is less than $1$. 
We will provide more details about the exact training procedure used to obtain the figure, in a later section. 
% \begin{figure}
% \centering
% \includegraphics[scale=0.3]{ideal}
% \hspace{1in}
% \includegraphics[scale=0.3]{learned}
% \caption{Figure on the left shows a Bayes optimal classifier for the data. Figure on the right shows the classifier obtained by minimizing the adversarial loss defined in Equation~\eqref{eqn:adv_obj}.}
% \label{fig:ideal_vs_learned}
% \end{figure}


\subsection{Standard training with increasing model complexity}
Before we conclude the section, we show how our results from Theorem~\ref{lem:equiv} can be used to explain an interesting phenomenon observed by \cite{madry2017towards}: even with standard risk minimization, complex networks result in more robust classifiers than simple networks. 
Define the standard and adversarial training objectives as
\[
\textbf{(standard) }\min_{f \in \mathcal{F}} R(f),
\]
\[
\textbf{(adversarial) } \min_{f \in \mathcal{F}} R(f) + \lambda G_{\text{adv}}(f).
\]
Recall in Theorem~\ref{lem:equiv} we showed that when $\mathcal{F}$ is the space of measurable functions, and if the Bayes optimal satisfies the margin condition, the minimizers of both these objectives have the same decision boundary, under the mild condition that $g(x)$ is Bayes optimal.
%We utilize this result to explain an interesting phenomenon observed by \cite{madry2017towards}: even with traditional training, complex networks result in more robust classifiers than simple networks. 
%
 
Let $\mathcal{F}$ be a small function class, such as the set of functions which can be represented using a particular neural network architecture. As we increase the complexity of $\mathcal{F}$, we expect the minimizer of $R(f)$ to move closer to a Bayes optimal classifier. Following Theorem~\ref{lem:minimizers}, since the minimizer of the adversarial training objective is also a Bayes optimal classifier, as we increase the complexity of $\mathcal{F}$ we expect the joint risk $R(f) + \lambda R_{\text{adv}}(f)$ to go down. Conversely, a similar explanation can be used to explain the phenomenon that performing adversarial training on complex networks results in classifiers with better classification risk. 
%This explanation can be extended to empirical risks over small hypothesis classes $\mathcal{F}$, where empirical risks $R_n(f), R_{n, \text{adv}}(f)$ have similar landscape as their population counterparts.
Figures~\ref{fig:depth_ERM},~\ref{fig:depth_pgd_gen} illustrate the two phenomena on MNIST and CIFAR10 datasets. More details about the experiments can be found in the Appendix.
%
\begin{figure}[H]
\centering     
\begin{minipage}[b]{0.48\textwidth}
\begin{subfigure}
{\includegraphics[width=0.48\textwidth]{plots/mnist.eps}}
{\includegraphics[width=0.48\textwidth]{plots/cifar.eps}}
\caption{\small{Behavior of joint $0/1$ risk of models obtained through traditional training, as we increase the model capacity. }}
\label{fig:depth_ERM}
\end{subfigure}
\end{minipage}
\hspace{0.15in}
\begin{minipage}[b]{0.48\textwidth}
\begin{subfigure}
{\includegraphics[width=0.485\textwidth]{plots/mnist_pgd_gen.eps}}
{\includegraphics[width=0.485\textwidth]{plots/cifar_pgd_gen.eps}}
\caption{\small{Behavior of classification $0/1$ risk of models obtained through adversarial training (with $\lambda = 1$), as we increase the model capacity.}}
\label{fig:depth_pgd_gen}
\end{subfigure}
\end{minipage}
\end{figure}
% \begin{figure}[!ht]
% \centering     
% \begin{subfigure}
% {\includegraphics[width=0.3\textwidth]{plots/convex}}
% \end{subfigure}
% \end{figure}

Before we conclude the section we point out that since in practice we optimize empirical risks instead of population risks, our explanations above are accurate only for smaller hypothesis spaces, where empirical risks and the corresponding population risks have similar landscapes. 



% \begin{itemize}
% \item Highlight the advantages of this formulation. How can we train this objective?
% \item Does $\lambda$ act as a parameter which trades off true risk and adversarial risk? Run some simulations where you have knowledge of $g(x)$.
% \item Talk about the choice of the norm.
% \item perform experiments on MNIST.
% \end{itemize}
% Some TODOs:
% \begin{itemize}
% \item \textit{Generalize the above result to any classification calibrated surrogate loss (see \citet{bartlett2006convexity} for definition).}
% \item \textit{What can we say about the minimizers of true risk and the objective in \eqref{eqn:objective_mod}, for a general hypothesis class $\mathcal{F}$? }
% \begin{itemize}
% \item \textit{If the minimizers of both the objectives are not related, what role does $\mathcal{R}_{\text{adv}}$ play?}
% \end{itemize}
% \item \textit{Does the relation between \eqref{eqn:objective_mod},\eqref{eqn:adv_obj} hold for any hypothesis class $\mathcal{F}$?} Looks like it should hold.
% \item \textit{What if $g$ is not Bayes optimal? Will the above results still hold?}
% If $g(x)$ is not Bayes optimal, then we can construct examples where the minimizers of true risk and \eqref{eqn:objective_mod} are not the same. It is also easy to see that \eqref{eqn:objective_mod} and \eqref{eqn:adv_obj} will not have the same set of minimizers.
% \end{itemize}


% \begin{figure}[!ht]   
% \subfigure[\label{fig:mnist_pgd} \small{{Performance of PGD training (with $\epsilon = 0.05$) on single hidden layer network with 400 hidden units.}}]{\includegraphics[width=0.4\textwidth, trim={0 0cm 0cm 0}, clip]{plots/mnist_pgd}}
% \hspace{0.1in}
% \subfigure[\label{fig:mnist_pgd} \small{{Example illustrating the behavior of minimizers of ERM.}}]{\includegraphics[width=0.4\textwidth, trim={0 0cm 0cm 0cm}, clip]{plots/convex}}
% \end{figure}
% \subsection{Toy Examples}
% In this section we consider simple examples which illustrate the salient aspects of true and adversarial risks.
% \paragraph{Concentric Circles.} Consider the following data generation process in $\mathbb{R}^2$ (see Figure \ref{fig:vc}). The probability distribution $\mathcal{P}$ is such that instances are distributed uniformly within the circle of radius $\sqrt{2}$. If an instance falls in the circle of radius $1$, then it is labeled `$+$', otherwise it is labeled as `$-$'.  
% \begin{figure}[H]
% \begin{center}
%  \includegraphics[width=0.25\textwidth]{concentric_example}
% \end{center}
% \caption{Concentric Circles. Figure shows samples generated using the data generation process described above.}
% \label{fig:vc}
% \end{figure}
% Let $g$ be the Bayes optimal classifier, which is given by 
% \[
% g(x) = \begin{cases}
% -1 \quad & \text{if} \|x\|_2 \geq 1\\
% 1 \quad & \text{otherwise}
% \end{cases}.
% \]
% Let hypothesis class $\mathcal{F}$ be the set of axis aligned squares, centered at origin. Let $f_s \in \mathcal{F}$ be a square of side $s$. The adversarial and true risks of $f_s$ are given by
% \[
% \mathcal{R}(f_s) = \begin{cases} 
% \frac{1}{2} - \frac{s^2}{2\pi} \quad & \text{if } s \leq \sqrt{2},\\
% \frac{s^2}{2\pi}-\frac{1}{2} + \frac{4}{\pi}\left(\cos^{-1}(s/2) - \frac{s}{2}\sqrt{1 - \frac{s^2}{4}}\right) \quad & \text{if } \sqrt{2} \leq s \leq 2,\\
% \frac{1}{2} - \frac{2}{\pi}\left(2\cos^{-1}(s/2\sqrt{2}) - \frac{s}{2}\sqrt{2-\frac{s^2}{4}}\right) \quad & \text{if } 2 \leq s \leq 2\sqrt{2},\\
% \frac{1}{2} \quad & \text{if } s \geq 2\sqrt{2}
% \end{cases}.
% \]
% \[
% \mathcal{R}_{\text{adv}}(f_s) \approx \begin{cases} 
% 4\epsilon s \quad & \text{if } s \leq 2,\\
% 8\epsilon\sqrt{2 - \frac{s^2}{4}} \quad & \text{if } 2 \leq s \leq 2\sqrt{2},\\
% 0 \quad & \text{if } s \geq 2\sqrt{2}
% \end{cases}.
% \]

% \paragraph{Gaussian Mixtures.} Consider the following generative model. $$p(y = 1) = p(y = 2) = 0.5, \ p(x|y = 1) = \mathcal{N}(-2, 1), p(x|y = 2) = \mathcal{N}(2, 4).$$ Let $g(x)$ be the Bayes optimal classifier and $\mathcal{F}$ be the set of linear classifiers $$\{f_{\theta}:\mathbb{R}\to \{1,2\}: f(x) = 2, \text{ if } x > \theta, f(x) =1 \text{ otherwise}\}.$$ $g(x)$ is given by 
% \[
% g(x) = \begin{cases}
% 1, \text{ if } -6.32 \leq x \leq -0.34\\
% 2, \text{ otherwise}
% \end{cases}.
% \]
% The true risk $\mathcal{R}(f_{\theta})$ is given by $$\mathcal{R}(f_{\theta}) = \frac{1}{2}\left(1 - \Phi(\theta + 2) + \Phi(\theta/2 - 1)\right).$$ This is minimized at $\theta = -0.34$.
% The adversarial risk is given by
% \[
% \mathcal{R}_{\text{adv}}(f_\theta) = \begin{cases}
% P_{x \sim D}(\theta \leq x \leq \min(\theta+\epsilon, -6.32))\quad &\text{if } \theta \in (-\infty , -6.32)\\
% P_{x \sim D}(\max(-6.32, \theta - \epsilon) \leq x \leq \theta)\quad &\text{if } \theta \in (-6.32, -0.34)\\
% P_{x \sim D}(\theta \leq x \leq \theta +\epsilon) \quad &\text{if } \theta \in (-0.34, \infty)\\
% 0 & \text{otherwise}
% \end{cases}.
% \]
% $\mathcal{R}_{\text{adv}}(f_\theta)$ is also minimized at $\theta = -0.34$. So, for any value of $\lambda$, Equation~\eqref{eqn:objective_mod} is minimized at $\theta = -0.34$.
% \paragraph{Simple vs. Complex Classes.} Assume that $g(x)$ is the Bayes optimal classifier. It is easy to see that $g(x)$ is a minimizer of both true and adversarial risks. We are now interested in knowing if there is any trade-off between adversarial and true risks as we increase the complexity of hypothesis space $\mathcal{F}$. \citet{fawzi2018analysis} vaguely claim that classifiers with high accuracy are less robust. However, according to our definition of robustness it is easy to see that this is not true. As we increase the complexity of $\mathcal{F}$, we can get better approximations of $g(x)$, which is a minimizer of both true and adversarial risks. As a result both true and adversarial risks can go down with increasing complexity of $\mathcal{F}$.

% The following example shows that complex decision boundaries can be more robust to adversarial perturbations than simple decision boundaries and at the same time have low true risk. However, the drawback of learning from complex function classes is the high sample complexity required for good generalization. 
% \begin{figure}[H]
% \begin{center}
%  \includegraphics[width=0.5\textwidth]{complex_adv}
% \end{center}
% \caption{The best linear classifier has very high adversarial risk, although it has $0$ true risk. Whereas the best quadratic classifier has very low adversarial and true risks.}
% \label{fig:complex_adv}
% \end{figure}


% In the special case when $g(x)$ is a Bayes optimal classifier and $\lambda = 1$, the above optimization problem can be rewritten as
% \begin{equation}
% \label{eqn:objective_mod_simplified}
% \argmin_{\theta \in \Theta} \mathbb{E}\left[\sup_{\begin{subarray}{c} \|\delta\|\leq \epsilon\end{subarray}} \mathbb{I}\left( g(x) = g(x+\delta) \wedge f_{\theta}(x+\delta) \neq g(x+\delta) \right)\right].
% \end{equation}
%The above objective has been studied in \citet{wang2016theoretical}.
% \paragraph{Optimization.} In practice we usually don't have access to the base classifier $g$. Assuming that $\epsilon$ is small and $g$ is a Bayes optimal classifier with margin atleast $\epsilon$, then Equation~\eqref{eqn:objective_mod} can be rewritten as
% \[
% \argmin_{\theta \in \Theta} \mathbb{E}_D\left[\mathbb{I}(f_\theta(x) \neq y)\right] + \lambda P(\mathcal{E}) \mathbb{E}_D\left[\left. \sup_{\begin{subarray}{c} \|\delta\|\leq \epsilon\end{subarray}} \mathbb{I}\left(  f_\theta(x+\delta) \neq y \right)  \right| \mathcal{E}\right],
% \]
% where event $\mathcal{E}$ is defined as $\mathcal{E} = \{f_{\theta}(x) = y\}$. 
% Note that when $\lambda = 1$ we retrieve the objective in Equation~\eqref{eqn:adv_obj}. 
% \begin{itemiz}
% \item Is it 
% \item \[\min_{\theta} \mathbb{E}_D\left[\mathbb{I}(f_\theta(x) \neq y)\right]\] \[\text{s.t. } \forall x \quad \left[\min_{\begin{subarray}{c} \delta \\ \text{s.t. } f(x) = g(x) = g(x+\delta),\\ g(x) \neq f(x+\delta)\end{subarray}} \|\delta\| \right] \geq \epsilon.\]
% \end{itemize}

==> meetings.tex <==
% \subsection{March $30$, 2018}
% Problems to look into:
% \begin{itemize}
% \item How to design attacks based on the current framework?
% \item How to defend against such attacks?
% \item How to train a model that is robust to adversarial attacks?
% \item If training a model from scratch is difficult, how can we improve a pre-trained model? Think of two cases here: a) we have black box access to $g$ b) $g$ is Bayes optimal.
% \item Remove the norm constraint the is usually used in defining adversarial perturbations. Instead use connected components in the ambient space of $g$ to define adversarial perturbations.
% \item Investigate if adversarial risk helps improve the generalization error. It looks like this should be the case. 
% \end{itemize}

==> related_work.tex <==
We now briefly review the existing literature on adversarial robustness.  Existing works define an adversarial perturbation at a point $x$, for a classifier $f$ as any perturbation $\delta$ with a small norm, measured w.r.t some distance metric, which changes the output of the classifier; that is $f(x+\delta) \neq f(x)$. Typically the distance metric is chosen to be an $L_p$ norm. Most of the existing techniques for adversarial training minimize the worst case error against all possible perturbations
\begin{equation}
\label{eqn:adv_obj}
\mathbb{E}_{(x,y) \sim \mathcal{P}}\left[\sup_{\delta: \norm{\delta}{} \leq \epsilon} \ell(f(x+\delta), y)\right].
\end{equation} 
\citet{carlini2017adversarial, goodfellow2014explaining, madry2017towards} use heuristics to approximately minimize the above objective. In each iteration of the optimization, these techniques first use heuristics to approximately solve the inner maximization problem and then compute a descent direction using the resulting maximizers. \citet{tsuzuku2018lipschitz} provide a training algorithm which tries to find large margin classifiers with small Lipschitz constants, thus ensuring robustness to adversarial perturbations. A recent line of work has focused on optimizing an upper bound of the above objective. \citet{raghunathan2018certified,zico} provide SDP and LP based upper bound relaxations of the objective, which can be solved efficiently for small networks. 
Since optimization of objective~\eqref{eqn:adv_obj} is difficult, \citet{sinha2017certifiable} proposed to optimize the following distributional robustness objective, which is a slightly weaker notion of robustness 
\begin{equation}
\label{eqn:dist_robust}
\min_{f} \max_{\mathcal{Q}: d(\mathcal{P}, \mathcal{Q}) \leq \epsilon} \mathbb{E}_{(x,y) \sim \mathcal{Q}}\left[\ell(f(x), y)\right],
\end{equation}
where $d(\mathcal{P},\mathcal{Q})$ is an appropriately chosen distance metric between probability distributions.

Another line of work on adversarial robustness has focused on studying adversarial risk from a theoretical perspective. These works characterize the robustness at a point $x$ in terms of how much perturbation a classifier can tolerate at a point, without changing its prediction
\begin{align}\label{eqn:fawzidef}
\quad r(x) = \min_{\delta \in \calS } \norm{\delta}{} \ \st \ \text{sign}(f(x)) \neq \text{sign}(f(x+\delta)),
\end{align}
where $\calS$ is some subspace. 
% Then, the goal is either to find a classifier $f$ which optimizes the worst-case radius\citep{tsuzuku2018lipschitz,uesato2018adversarial,wang2016theoretical}
% \[
% \text{(Worst Case) } \quad \min_{f \in \mathcal{F}} \mathbb{E}\left[\ell_{0-1}(y, f(x))\right] \quad \st \  r(x) \geq \delta, \forall x
% \]
The expected adversarial radius is defined as $\mathbb{E}[r(x)]$ \citep{fawzi2018analysis,2018arXiv180208686F,franceschi2018robustness}.
%Note that the worst-case robustness is a very strong and restrictive requirement. 
%To give results in this setting requires making unreasonable assumptions such as $f:\mathbb{R}^p \rightarrow \{1, \dots L\}$ being continuous everywhere.
%and learning a \emph{finer} representation than the original label generating model  \cite{wang2016theoretical}. 
%Several recent works analyze this incorrect definition of adversarial perturbations and  
\citet{fawzi2018analysis} theoretically study the expected adversarial radius, for any classifier $f$ and suggest that there is a trade-off between adversarial robustness and the prediction accuracy ($\mathbb{P}(y = f(x))$). Specifically, their results suggest that if the prediction accuracy is high then $\mathbb{E}[r(x)]$ could be small. 
%Under the assumption that the covariates are generated by a generative model which maps latent vectors to data points in the distribution, \cite{2018arXiv180208686F} give conditions under which $\mathbb{E}[r(x)]$ can be arbitrarily small for any classifier $f$. 

A careful inspection of adversarial perturbation and adversarial radius defined in Equations~\eqref{eqn:adv_obj},\eqref{eqn:fawzidef} brings into light the issues with these definitions.
A major issue with these definitions is that they assume the response variable $y$ is smooth in a neighborhood of $x$, which may not be true in general. For example, if a perturbation $\delta$ is such that ``true label'' at $x$ is not same as the ``true label'' at $x+\delta$ then the perturbation shouldn't be considered as adversarial. This incorrect definition of adversarial perturbation has resulted in several recent works claiming that there exists a ``trade-off between adversarial robustness and generalization''. An evidence against these claims is the fact that in image classification tasks, humans are robust classifiers with low error rate.

To be more concrete, consider two points $(x_1,1)$ and $(x_1+\delta,-1)$ which are close. Then for any classifier $f$ to be correct at the two points, it needs to change its score for the two points over a small interval, which would mean that $r(x_1)$ would be very small. More importantly, if the distribution $\mathcal{P}$ is such that there is a huge probability mass on ``boundary'' points such as $x_1$, then in order to have high accuracy, the classifier will have to change its score, leading to a small $\mathbb{E}[r(x)]$, which creates the illusion of a trade-off between adversarial robustness and generalization. This illusion arises because of the above definitions of adversarial perturbation which consider the perturbation $\delta$ at $x$ to be adversarial. On the contrary, $\delta$ shouldn't be considered adversarial because the true label at $x_1+\delta$ is not the same as the label at $x_1$. This confusion motivates the need of giving a clear definition of an adversarial perturbation, the corresponding adversarial risk, and then studying these quantities. 
%Most of the existing inconsistencies occur because of incorrect definitions of adversarial loss and adversarial radius. Consider the case of image classification, where examples of adversarial attacks involve giving an image $x$, which both humans and the model classify correctly, but a tiny perturbation which is imperceptible to a human is classified incorrectly by the model. Note that the use of the notion of a human is key to defining an adversarial perturbation. For example, if there was an image on which both humans and models disagreed, then perturbations of such an image are not ``adversarial''. 

% \subsection{Background}
% There  are three different robust optimization formulations commonly used to learn models that are robust to adversarial attacks.
% \paragraph{Local Adversarial Robustness.}
% \begin{equation}
% \label{eqn:advrs_robust}
% \min_{\theta} \mathbb{E}_{(x,y) \sim P}\left[\max_{\delta: \|\delta\| \leq \epsilon}\ell(f_\theta(x + \delta), y)\right],
% \end{equation}
% where $P$ is the true data distribution and $f_\theta: \mathbb{R}^p \to \mathbb{R}^{|L|}$ is a score based classifier.  
% % Suppose the loss $\ell$ is $0/1$ loss. Then the above objective can be rewritten as
% % \[
% % \min_{\theta} \underbrace{\mathbb{E}_{(x,y) \sim P}\left[\ell(f_\theta(x), y)\right]}_{\text{True Risk}} + P(y = \argmax_{i}[f_\theta(x)]_i)\underbrace{\mathbb{E}_{(x,y) \sim P}\left[\max_{\tilde{x}: d(x, \tilde{x}) \leq \epsilon} \ell(f_\theta(\tilde{x}), y)\left|y = \argmax_{i}[f_\theta(x)]_i\right.\right]}_{\text{Adversarial Risk}}.
% % \]
% \paragraph{Distributional Robustness.}
% \begin{equation}
% \label{eqn:dist_robust}
% \min_{\theta} \max_{Q: d(P, Q) \leq \epsilon} \mathbb{E}_{(x,y) \sim Q}\left[\ell(f_\theta(x), y)\right],
% \end{equation}
% where $d(P,Q)$ is an appropriately chosen distance metric between probability distributions. \citet{sinha2017certifiable} optimize this objective to learn robust classifiers. Distributional robustness looks like a weaker notion than adversarial robustness; that is, there could be functions $f_{\theta}$ which are distributionally robust but not adversarially robust.
% \paragraph{Stability.}
% \begin{equation}
% \label{eqn:stability_robust}
% \min_{\theta} \mathbb{E}_{(x,y) \sim P}\left[\ell(f_\theta(x), y)\right] \quad \text{s.t. } \max_{x} \max_{\delta: \|\delta\| \leq \epsilon} d(f_\theta(x), f_\theta(x+ \delta)) \leq \eta,
% \end{equation}
% where $d$ is a distance metric.
% The above constraint is usually satisfied if $f_{\theta}$ is a Lipschitz function
% \[
% d(f_{\theta}(x_1), f_{\theta}(x_2)) \leq C \|x_1- x_2\| \quad \forall x_1, x_2.
% \]
% Lipschitzness of $f_{\theta}(x)$ together with margin separation ($[f_{\theta}(x)]_{y} - \max_{j \neq y} [f_{\theta}(x)]_{j} \geq \epsilon > 0$) are sufficient to make the objective in Equation\eqref{eqn:advrs_robust} small; that is, they are sufficient to ensure robustness of a classifier to adversarial perturbations. \citet{tsuzuku2018lipschitz} provide a training algorithm which tries to find large margin classifiers with small Lipschitz constants, thus ensuring robustness to adversarial perturbations.

% \begin{remark}
% What should be the goal of adversarial robustness? Is Equation~\eqref{eqn:advrs_robust} the right problem to solve? To answer these questions, we should first formally define adversarial attacks and attack model. How good is the current attack model? It'd be good to have some applications in mind.  
% One example is the self-driving car where an image from a camera must  be correctly classified according to the type of object in its view, irrespective of aspects such as the angle of its vision and image imperfections.
% %See \citet{HuangKWW16, BastaniILVNC16} and references therein for ideas on how people tried to formalize adversarial robustness.
% \end{remark}
% \begin{remark}
% We couldn't think of any real applications where the current attack model is valid. For example, the current model assumes $\ell_{\infty}$ perturbations and importantly assumes that the perturbations are imperceptible to humans. Why should an adversary be restricted to making imperceptible changes?
% \end{remark}
% \begin{remark}[Bayes Estimator]
% \textcolor{red}{TODO:} Try to investigate if Bayes estimators are inherently robust to adversarial perturbations.
% \end{remark}
% \begin{remark}
% Many of the existing techniques train a network for some adversarial perturbation $\epsilon$. Will these techniques perform well on test data with perturbations more than $\epsilon$?
% \end{remark}
%



==> risk_adversarial.tex <==
\section{Standard vs Adversarial Risk: A Dichotomy?}
In the previous sections, we studied the properties of adversarial risk when $g(x)$ is either the Bayes Optimal or the stochastic label $y$. In particular, we showed that when the Bayes optimal($g(x)$) is unique, $g(x)$ is the \emph{unique} minimizer of both the standard and adversarial risk. This in a sense establishes the \emph{consistency} of the two risks.

In this section, we go a step further and study the consequences of the bayes optimal being under approximation or identification issues. Approximability issues can arise because of a number of reasons such as (1) Finite-sample approximation of standard risk (2) Optimizing the standard risk over a restricted function class. In practice, one typically has access to only finite samples and decides the model-class(such as linear) apriori, hence, both these scenarios occur quite commonly.

Similarly, when the data is separable, or lies in a low-dimensional manifold, then the Bayes optimal is not unique. Then, a natural task is to study is the behavior of adversarial risk of one \emph{optimal} classifier to the other.

We study these questions theoretically under a synthetic mixture model where the data for each class is generated from a different mixture component. In this example, the distribution of $x$ conditioned on $y$ follows a normal distribution: $x | y \sim \calN(y \theta^*, \sigma^2 \calI_p)$, where $\calI_p \in \mathbb{R}^{p \times p}$ is the identity matrix and $\mathbb{P}(y=1) = \mathbb{P}(y = -1) = \half$. Note that in this setting $x  \mapsto  x^T\theta^*$ is a Bayes optimal classifier. Firstly, we present a result which characterizes the behavior of standard and adversarial risks in this model.

\begin{theorem}\label{thm:mixture}
Suppose the perturbations are measured w.r.t $L_{\infty}$ norm. Let $w \in \real^p$ be a linear separator and moreover suppose the base classifier $g(x)$ is the Bayes optimal decision rule. Then, for any linear classifier $f_w(x) = w^T x$, we have that
\begin{enumerate}
\item $ R_{0-1}(f_w) = \Phi\paren{ - \frac{w^T \tparam}{\sigma \norm{ w}{2}}},$
\item $ G_{\text{adv}, 0-1}(f_w) = \Phi \paren{ \frac{\norm{w}{1}\epsilon - w^T \theta^*}{\sigma \norm{w}{2}}}, $
\item $ R_{\text{adv},0-1}(f_w) \leq \Phi \paren{ \frac{\norm{w - \theta^*}{1}\epsilon - (w - \theta^*)^T \theta^*}{\sigma \norm{w - \tparam}{2}}}$,
\end{enumerate}
where $\Phi(\cdot)$ is the CDF of the standard normal distribution.
\end{theorem}

\subsection{Calibration of Standard and Adversarial Risk}
In this section, we go a step further and explore if the two risk functions are \emph{calibrated}, \ie \emph{does {approximately} minimizing the standard risk always lead to small adversarial risk?} To this end, suppose the mean of the Gaussian components is $s$-sparse; that is, $\tparam$ has $s$ non-zero entries. In this setting, the Bayes optimal classifier $x \mapsto \tparam^T x$ depends only on a few features and there are a lot of irrelevant features \wrt classifying the data. Our next result shows that there exist linear separators which achieve near optimal classification accuracy, but their adversarial risk is high, even for an adversarial perturbation of size $\frac{1}{\sqrt{p-s}}$. 

\begin{lemma}\label{cor:sparse}
Let $\theta^*$ be $s$-sparse with non-zeros in the first $s$ coordinates. Let $w \in \mathbb{R}^p$ be a linear separator such that $w_{1:s} = \theta^*_{1:s}$, $w_{s+1:p} = [ \frac{\pm1}{\sqrt{p-s}},\ldots,\frac{\pm1}{\sqrt{p-s}}]$. Then, there exists a constant $C$ such that if $\norm{\tparam}{2} \geq C$ and $\sigma =1$, the excess risk of $f_w$ is small; that is, $R_{0-1}(f_w) - R^*_{0-1} \leq  0.02$, where $R^*_{0-1}$ is the risk of the Bayes optimal classifier. However, even for a small enough perturbation $\epsilon \geq \frac{2\|\theta^*\|^2_2}{\sqrt{p-s}}$ w.r.t $L_{\infty}$ norm, the adversarial risk satisfies \[ R_{adv,0-1}(f_w) \geq 0.95 .\]
\end{lemma}

To give some intuition, note that the constructed classifier $w$ has a very small mass on the irrelevant features, hence the classification error is low, but since there are a lot of such irrelevant features, there exists adversarial perturbations only on the subspace of irrelevant features, such that they don't change the prediction of the Bayes classifer, but they change the prediction of $w$.


\subsection{Optimizing Standard Risk over Restricted Function Class}
Next, we study the effect of minimizing the standard risk over restricted function classes $\Theta$, instead over the space of all measurable functions. Consider the restricted hypothesis class, $\Theta$ of all vectors which are non-zero in the top-$s$ co-ordinates, \ie $\Theta = \{ \theta \in \real^p | ~ \theta_i = 0 \ \forall i > s+1 \}$. Our next result shows that the there exists mixture models such that the \emph{exact} minimizer of the standard risk over this restricted hypothesis class is \emph{not} the minimizer of the adversarial risk, even for perturbations as small as $\frac{1}{\sqrt{p-1}}$.

\begin{lemma}\label{lem:functionClass}
Consider the gaussian mixture model, $x | y \sim \calN(y \tparam,I_p)$ where $\tparam = [1,\frac{1}{\sqrt{p-1}},\frac{1}{\sqrt{p-1}},\ldots,\frac{1}{\sqrt{p-1}}]^T$ and let $\tilde{\theta} = \argmin_{\theta \in \Theta} R_{0-1}(f_{\theta})$ be the minimizer of the standard risk when restricted to $\Theta$. Then, even for a small enough perturbation of $\epsilon \geq \frac{1}{\sqrt{p-1}}$ \wrt $L_{\infty}$ norm, there exists a vector $m \in \Theta$ such that,
\[ R_{0-1}(f_{\tilde{\theta}}) < R_{0-1}(f_m) ~~ \emph{but} ~~ R_{adv,0-1}(f_{\tilde{\theta}}) > R_{adv,0-1}(f_m). \]
\end{lemma}


\subsection{Multiple Bayes Optimal}
In our previous examples, we always assumed that the Bayes Optimal is unique. Our next example studies when there are multiple Bayes optimal. Then, we answer the question of whether one bayes optimal solution adversarially robust to the other. More importantly, do current training algorithms converge to such bayes optimal solutions which are non-robust to other bayes-optimal solutions. \\
Suppose our data comes from low dimensional Gaussians embedded in a high-dimensional space, \ie suppose $\norm{\tparam}{0} = s \ll p$ and the covariance matrix $D$ of the conditional distributions $x|y$ is diagonal with $i^{th}$ diagonal entry $D_{ii} = \sigma^2~\text{if}~\theta_i^* \neq 0, 0~\text{otherwise}$. Observe the subtle difference between this setting and sparse mixture model. In particular, in the previous example, the data is inherently high-dimensional, but with only a few relevant discriminatory feature; on the contrary, here the data lies on a low dimensional manifold of a high dimensional subspace.

In this setting, we want to study the adversarial risk of classifier obtained by minimizing calibrated convex surrogates~\citep{bartlett2006convexity} of the 0-1 loss using iterative methods such as gradient descent.
\begin{figure}[H]
\centering
\includegraphics[scale=0.35]{non-robust.png}
\caption{\small{One-dimensional mixture embedded in a 2-D space. Observe the classifier that is nearly parallel to the $x_1$ axis. Despite having low true risk, it will have high adversarial risk for a small $\epsilon$}}
\label{fig:robust}
\end{figure}

\begin{lemma}\label{cor:surr}
Let $\tparam$ be such that $\norm{\tparam}{2} \geq C$, for some constant $C$. Let $\epsilon \geq \frac{2\|\theta^*\|^2_2}{\sqrt{p-s}}$ and $\ell$ be any convex calibrated surrogate loss $\ell(f_\theta, (y,x)) = \phi(y\theta^Tx)$. Then gradient descent on $R(f_\theta)$ with random initialization using a Gaussian distribution with covariance $\frac{1}{\sqrt{p-s}}\calI_p$ converges to a point $\widehat{\theta}_{GD}$ such that with high probability,
\[ 
 R_{0,1}(f_{\widehat{\theta}_{GD}}) = 0~~ \text{but} ~~ R_{adv,0-1}(f_{\widehat{\theta}_{GD}}) \geq 0.95, \]
 where $R_{adv,0-1}(\cdot)$ is the adversarial risk measured \wrt $\tparam$.
\end{lemma}

Note that Lemma~\ref{cor:surr} raises the vulnerability of current training procedures by showing that they can lead to solutions which have high adversarial risk. Moreover, observe that increasing $p$ results in classifiers that are less robust; even a $O(1/\sqrt{p-s})$ perturbation can create adversarial examples with respect to another Bayes optimal. 

All our results before show that standard risk minimization is inherently insufficient in providing robustness when either  the minimization is inexact or the risk has multiple minima. This suggests the need of minimizing the joint risk or adverarially training our models.
% In this section, we go a step further and explore if the two risk functions are \emph{calibrated}, \ie \emph{does {approximately} minimizing the standard risk always lead to small adversarial risk?} Note that this is important to understand as in order to identify     \ie \emph{do classifiers which have very small 0-1 risk also necessarily have small adversarial risk?}   minimize the 0-1 risk but perfoer

% Having formally defined adversarial risk,id th we next consider concrete examples to illustrate the difference between the new and existing definitions of adversarial risk and study their behavior in high dimensional spaces. We consider the following two data models: (1) a mixture model, where the data for each class is generated from a different mixture component, and (2) a separable dataset on a bounded domain. 

% \subsection{Mixture Model}
% In this example, the distribution of $x$ conditioned on $y$ follows a normal distribution: $x | y \sim \calN(y \theta^*, \sigma^2 \calI_p)$, where $\calI_p \in \mathbb{R}^{p \times p}$ is the identity matrix and $\mathbb{P}(y=1) = \mathbb{P}(y = -1) = \half$. 
% %\textcolor{red}{TODO: This is a degenerate Gaussian. Be careful when you use it somewhere. Also define what $\calI_r$ exactly is.}
% With a slight overload of notation, we let $G_{adv,0-1}(f) = \Exp \sqprn{\max \limits_{\delta: \norm{\delta}{} \leq \epsilon} \ell_{0-1}(f(x+\delta),y)}$ be the definition of adversarial risk used in existing works on adversarial training. 
% Note that in this setting $x  \mapsto  x^T\theta^*$ is a Bayes optimal classifier. Firstly, we present a result which characterizes the behavior of standard and adversarial risks in this model.

% \begin{theorem}\label{thm:mixture}
% Suppose the perturbations are measured w.r.t $L_{\infty}$ norm. Let $w \in \real^p$ be a linear separator and moreover suppose the base classifier $g(x)$ is the Bayes optimal decision rule. Then, for any linear classifier $f_w(x) = w^T x$, we have that
% \begin{enumerate}
% \item $ R_{0-1}(f_w) = \Phi\paren{ - \frac{w^T \tparam}{\sigma \norm{ w}{2}}},$
% \item $ G_{\text{adv}, 0-1}(f_w) = \Phi \paren{ \frac{\norm{w}{1}\epsilon - w^T \theta^*}{\sigma \norm{w}{2}}}, $
% \item $ R_{\text{adv},0-1}(f_w) \leq \Phi \paren{ \frac{\norm{w - \theta^*}{1}\epsilon - (w - \theta^*)^T \theta^*}{\sigma \norm{w - \tparam}{2}}}$,
% \end{enumerate}
% where $\Phi(\cdot)$ is the CDF of the standard normal distribution.
% \end{theorem}

% Before delving into different kinds of mixtures, we first take a step back and use Theorem~\ref{thm:mixture} to highlight the differences between the old definition of adversarial risk $G_{adv,0-1}(f)$, and our proposed definition $R_{adv,0-1}(f)$. Specifically, we first show that the Bayes Optimal classifier need not be the minimizer of $G_{\text{adv}, 0-1}(f)$. 


%  \begin{lemma}\label{cor:nobayes}
% Suppose $\tparam = [1,\frac{1}{\sqrt{p-1}},\frac{1}{\sqrt{p-1}},\ldots,\frac{1}{\sqrt{p-1}}]^T$. Let $\tilde{\theta} = [1,0,0,\ldots,0]^T$. Then 
% \[ G_{\text{adv}, 0-1}(f_{\tilde{\theta}}) < G_{\text{adv}, 0-1}(f_{\tparam}) \] 
%  \end{lemma}
% % This shows that there exist classifiers with smaller adversarial risk than Bayes optimal classifier and shows that minimizing $G_{\text{adv}, 0-1}$ need not result in a classifier with optimal classification risk. We study this phenomenon more formally in Section~\ref{sec:adv_training}.
% % Our next result shows that when $\theta^*$ is $s$-sparse, one can easily find classifiers which achieve high adversarial risk, but low true risk.

% \paragraph{Sparse Mixtures.} Suppose the mean of the Gaussian components is $s$-sparse; that is, $\tparam$ has $s$ non-zero entries. In this setting, the Bayes optimal classifier $x \mapsto \tparam^T x$ depends only on a few features and there are a lot of irrelevant features \wrt classifying the data. Our next result shows that there exist linear separators which achieve near optimal classification accuracy, but their adversarial risk is high, even for an adversarial perturbation of size $\frac{1}{\sqrt{p-s}}$. 

% \begin{lemma}\label{cor:sparse}
% Let $\theta^*$ be $s$-sparse with non-zeros in the first $s$ coordinates. Let $w \in \mathbb{R}^p$ be a linear separator such that $w_{1:s} = \theta^*_{1:s}$, $w_{s+1:p} = [ \frac{\pm1}{\sqrt{p-s}},\ldots,\frac{\pm1}{\sqrt{p-s}}]$. Then, there exists a constant $C$ such that if $\norm{\tparam}{2} \geq C$ and $\sigma =1$, the excess risk of $f_w$ is small; that is, $R_{0-1}(f_w) - R^*_{0-1} \leq  0.02$, where $R^*_{0-1}$ is the risk of the Bayes optimal classifier. However, even for a small enough perturbation $\epsilon \geq \frac{2\|\theta^*\|^2_2}{\sqrt{p-s}}$ w.r.t $L_{\infty}$ norm, the adversarial risk satisfies \[ R_{adv,0-1}(f_w) \geq 0.95 .\]
% \end{lemma}

% To give some intuition, note that the constructed classifier $w$ has a very small mass on the irrelevant features, hence the classification error is low, but since there are a lot of such irrelevant features, there exists adversarial perturbations only on the subspace of irrelevant features, such that they don't change the prediction of the Bayes classifer, but they change the prediction of $w$.

In the sparse setting, we showed the existence of a classifier which has very high adversarial risk, but low classification risk. However, merely showing the existence of such classifiers is not enough. A more pressing question is whether our current training algorithms converge to such classifiers. In our next example, we explore this question.

\paragraph{Low-Dimensional Embeddings.} Suppose our data comes from low dimensional Gaussians embedded in a high-dimensional space, \ie suppose $\norm{\tparam}{0} = s \ll p$ and the covariance matrix $D$ of the conditional distributions $x|y$ is diagonal with $i^{th}$ diagonal entry $D_{ii} = \sigma^2~\text{if}~\theta_i^* \neq 0, 0~\text{otherwise}$. Observe the subtle difference between this setting and sparse mixture model. In particular, in the previous example, the data is inherently high-dimensional, but with only a few relevant discriminatory feature; on the contrary, here the data lies on a low dimensional manifold of a high dimensional subspace.

In this setting, we want to study the adversarial risk of classifier obtained by minimizing convex surrogates of the 0-1 loss using iterative methods such as gradient descent.
\begin{figure}[H]
\centering
\includegraphics[scale=0.35]{non-robust.png}
\caption{\small{One-dimensional mixture embedded in a 2-D space. Observe the classifier that is nearly parallel to the $x_1$ axis. Despite having low true risk, it will have high adversarial risk for a small $\epsilon$}}
\label{fig:robust}
\end{figure}

\begin{lemma}\label{cor:surr}
Let $\tparam$ be such that $\norm{\tparam}{2} \geq C$, for some constant $C$. Let $\epsilon \geq \frac{2\|\theta^*\|^2_2}{\sqrt{p-s}}$ and $\ell$ be any convex surrogate loss $\ell(f_\theta, (y,x)) = \phi(y\theta^Tx)$. Then gradient descent on $R(f_\theta)$ with random initialization using a Gaussian distribution with covariance $\frac{1}{\sqrt{p-s}}\calI_p$ converges to a point $\widehat{\theta}_{GD}$ such that with high probability $R_{adv,0-1}(f_{\widehat{\theta}_{GD}}) \geq 0.95$.
\end{lemma}

Note that Lemma~\ref{cor:surr} raises the vulnerability of current training procedures by showing that they can lead to solutions which have high adversarial risk. Moreover, observe that increasing $p$ results in classifiers that are less robust; even a $O(1/\sqrt{p-s})$ perturbation can create adversarial examples with respect to the Bayes optimal. 


%The above results suggest that there is an explicit need to design training methods to minimize the joint risk. In the later sections we study how to optimize the joint risk via adversarial training, and highlight its additional saliencies.

% In this section, we will discuss some drawbacks in the results of \citet{fawzi2018analysis} and present some potentially interesting results that even contradict \citet{fawzi2018analysis}.

% First, recall that \citet{fawzi2018analysis} derive an upper bound on adversarial robustness for a given classifier. Specifically, they say that under some assumptions on the classifier $f$, $\rho_{adv}(f)$ (which is the norm of minimum perturbation required to flip the output of the classifier, in expectation over all datapoints in the underlying distribution) is not any larger than a term that grows with the  risk of the classifier and the inter-class distance. First, note that this is not a counter-intuitive result:   if we allow the classifier to have high risk, the classifier could simply output the same label on all datapoints and hence be robust to perturbations that try to flip its output. On the other hand, when the classifier faithfully outputs the true labels, if the inter-class distance is very small, smaller perturbations are likely to change the classifier's output.

% \begin{figure}[H]
% \centering
% \includegraphics[scale=0.4]{high-dim.png}
% \caption{A low risk, non-robust classifier for a high-dimensional distribution. As the spheres go farther apart and as $D$ increases, we can find classifiers that become more and more parallel to the $x_1$ axis)}
% \label{fig:high-dim}
% \end{figure}


% \subparagraph{Extension to non-low-manifold case}

% Is the above phenomenon limited to distributions on lower dimensional manifolds? To answer this question, consider a setting where the two classes are situated in uniform D-dimensional spherical distributions of radius $1$ centered at $x_1 = \gamma + 0.5$ and $x_1 = -\gamma - 0.5$ as shown in Figure~\ref{fig:high-dim}. The key idea is that, as these spheres go farther and farther apart from each other, we can find separators that are lesser and lesser robust. We formalize this in the following theorem .



% \begin{theorem}
% Assume we restrict ourselves to a space of classifiers whose $\ell_2$ norm is bounded by $\lambda$ (a value that is typically more of a constant compared to the dimensionality $D$). Then, there exists a classifier in this space that achieves zero risk with a margin of $1$ on all data points, and is susceptible to $\ell_\infty$ attacks of magnitude as small as $O\left (\frac{1+\lambda}{\frac{1+0.5 \lambda}{\gamma+0.5} + \sqrt{(D-1) \left( \lambda^2 - \frac{(1+0.5 \lambda)^2}{(\gamma+0.5)^2} \right)}}\right)$
% \end{theorem}

% \subparagraph{Remarks.} 
% \begin{itemize}
% \item Unlike the previous theorem, here we only show the existence of a non-robust classifier, not that gradient descent will necessarily learn it. 
% \item Observe that as $D$ increases, the robustness decreases rapidly!
% \end{itemize}

\subsection{Standard training with increasing model complexity}
Before we conclude the section, we show how our results from Theorem~\ref{lem:equiv} can be used to explain an interesting phenomenon observed by \cite{madry2017towards}: even with standard risk minimization, complex networks result in more robust classifiers than simple networks. 
Define the standard and adversarial training objectives as
\[
\textbf{(standard) }\min_{f \in \mathcal{F}} R(f),
\]
\[
\textbf{(adversarial) } \min_{f \in \mathcal{F}} R(f) + \lambda G_{\text{adv}}(f).
\]
Recall in Theorem~\ref{lem:equiv} we showed that when $\mathcal{F}$ is the space of measurable functions, and if the Bayes optimal satisfies the margin condition, the minimizers of both these objectives have the same decision boundary, under the mild condition that $g(x)$ is Bayes optimal.
%We utilize this result to explain an interesting phenomenon observed by \cite{madry2017towards}: even with traditional training, complex networks result in more robust classifiers than simple networks. 
%
 
Let $\mathcal{F}$ be a small function class, such as the set of functions which can be represented using a particular neural network architecture. As we increase the complexity of $\mathcal{F}$, we expect the minimizer of $R(f)$ to move closer to a Bayes optimal classifier. Following Theorem~\ref{lem:minimizers}, since the minimizer of the adversarial training objective is also a Bayes optimal classifier, as we increase the complexity of $\mathcal{F}$ we expect the joint risk $R(f) + \lambda R_{\text{adv}}(f)$ to go down. Conversely, a similar explanation can be used to explain the phenomenon that performing adversarial training on complex networks results in classifiers with better classification risk. 
%This explanation can be extended to empirical risks over small hypothesis classes $\mathcal{F}$, where empirical risks $R_n(f), R_{n, \text{adv}}(f)$ have similar landscape as their population counterparts.
Figures~\ref{fig:depth_ERM},~\ref{fig:depth_pgd_gen} illustrate the two phenomena on MNIST and CIFAR10 datasets. More details about the experiments can be found in the Appendix.
%
\begin{figure}[H]
\centering     
\begin{minipage}[b]{0.48\textwidth}
\begin{subfigure}
{\includegraphics[width=0.48\textwidth]{plots/mnist.eps}}
{\includegraphics[width=0.48\textwidth]{plots/cifar.eps}}
\caption{\small{Behavior of joint $0/1$ risk of models obtained through traditional training, as we increase the model capacity. }}
\label{fig:depth_ERM}
\end{subfigure}
\end{minipage}
\hspace{0.15in}
\begin{minipage}[b]{0.48\textwidth}
\begin{subfigure}
{\includegraphics[width=0.485\textwidth]{plots/mnist_pgd_gen.eps}}
{\includegraphics[width=0.485\textwidth]{plots/cifar_pgd_gen.eps}}
\caption{\small{Behavior of classification $0/1$ risk of models obtained through adversarial training (with $\lambda = 1$), as we increase the model capacity.}}
\label{fig:depth_pgd_gen}
\end{subfigure}
\end{minipage}
\end{figure}
% \begin{figure}[!ht]
% \centering     
% \begin{subfigure}
% {\includegraphics[width=0.3\textwidth]{plots/convex}}
% \end{subfigure}
% \end{figure}

Before we conclude the section we point out that since in practice we optimize empirical risks instead of population risks, our explanations above are accurate only for smaller hypothesis spaces, where empirical risks and the corresponding population risks have similar landscapes. 


